Domain-Specific Language Model Pretraining for Biomedical Natural Language Processing

Pretraining large neural language models, such as BERT, has led to impressive gains on many natural language processing (NLP) tasks. However, most pretraining efforts focus on general domain corpora, such as newswire and Web. A prevailing assumption is that even domain-specific pretraining can benefit by starting from general-domain language models. In this paper, we challenge this assumption by showing that for domains with abundant unlabeled text, such as biomedicine, pretraining language models from scratch results in substantial gains over continual pretraining of general-domain language models. To facilitate this investigation, we compile a comprehensive biomedical NLP benchmark from publicly-available datasets. Our experiments show that domain-specific pretraining serves as a solid foundation for a wide range of biomedical NLP tasks, leading to new state-of-the-art results across the board. Further, in conducting a thorough evaluation of modeling choices, both for pretraining and task-specific fine-tuning, we discover that some common practices are unnecessary with BERT models, such as using complex tagging schemes in named entity recognition (NER). To help accelerate research in biomedical NLP, we have released our state-of-the-art pretrained and task-specific models for the community, and created a leaderboard featuring our BLURB benchmark (short for Biomedical Language Understanding & Reasoning Benchmark) at https://aka.ms/BLURB.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> cover-letter.tex <==
Dear Professor Insup Lee,

Please find attached the revised version for our paper "Domain-Specific Language Model Pretraining for Biomedical Natural Language Processing". We are grateful to the insightful comments and suggestions by the reviewers and the Associate Editor. We have addressed all the required changes in this revision, prior to the January 31st deadline for the special issue on Biomedical NLP. 

Below, we summarize the changes in the revision and answer reviewers' questions.

Areas of improvement:

> 1. The claim that the direct domain specific pre-training yields better embedding and that continual pre-training is harmful are not *directly* proved. Reviewers suggest further experiments to explore this aspect:
    a. Is there a way to avoid local minima in pre-training while retaining general domain semantics?  (A reviewer recommends ways to address this question.)
    b. Is there a way to further analyze and demonstrate differences in embeddings for biomedical domain for the two ways of pre-training? A reviewer suggests studying embeddings for 15-20 biomedical terms with their corresponding morphological structure (hyper-ten-sion) 

1a: Thanks to the suggestion by reviewer 3, we conducted additional experiments demonstrating conclusively that pretraining on general-domain confers no benefit for biomedical NLP. See Table 9 for results. Specifically, we used the PubMed vocabulary, pretrained on Wiki + Books, then continued pretraining on PubMed (second column). The results are actually slightly worse than continual pretraining from the standard BERT with general-domain vocabulary (first column; BioBERT), and significantly worse than pretraining from scratch (fourth column). By running pretraining from scratch even with half of the compute (third column), the results are already comparable to BioBERT. Further pretraining produces additional gain.

1b: In Table 1, we added word-piece tokenization in various vocabularies for 17 biomedical terms. PubMedBERT vocabulary contains all these terms, whereas mixed-domain vocabularies often have to shatter them into word pieces with little biomedical relevance. Note that a BERT vocabulary is essentially a fixed-size collection of most frequent word pieces in the pretraining corpus, and the BERT tokenization does not necessarily conform with standard morphological structure in linguistics.

> 2. Characterize the time spent building a from-scratch model versus a continual model since pre-training is expensive and has a significant carbon footprint. For instance, how long does one need to train from scratch to achieve the same score as BioBERT? Some kind of time-versus-performance trade-off would be good to understand this aspect.

2: In our experiments, continual pretraining and pretraining from scratch used the same amount of total compute (equivalent to 2M BERT steps with batch size 256), so their comparison is head-to-head. Additionally, in Table 9, we added the results by pretraining from scratch with half of the compute (1M BERT steps; third column), which are already comparable to BioBERT and slightly better than continual pretraining with PubMed vocabulary (first and second columns), thus demonstrating that pretraining on general-domain text confers no advantage for biomedical pretraining. Note that pretraining only needs to be conducted once and the resulting PubMedBERT models can be used in a variety of biomedical applications.

> 3. Paper should be made more succinct by eliminating redundancy in introductory sections 1,2,3. Please use the IMRD (Intro, Methods, Results, and Discussion) format to avoid redundancy and to bring clarity to the presentation.

We eliminated redundancy in the original sections 1-3 and adopted the IMRD format. Thanks for the suggestion, the presentation is much clearer now.

> 4. Examples on how the updated vocabulary helped the NLP tasks alongside table 7.

We added Table 8, which shows that the input length is substantially shorter with an in-domain vocabulary, which generally makes learning for downstream tasks easier. 

We added Figure 3, which gives examples on how the in-domain vocabulary enables PubMedBERT to learn better attention patterns and fix errors of BioBERT.

Reviewer 1:

Thanks for the encouraging review and suggestions! Evaluating on clinical NLP is indeed an important next step. As mentioned in the paper, we focus on domain-specific pretraining in biomedical publications. Since clinical notes are quite different from PubMed papers, we intend to investigate the clinical domain separately in future work. Preliminary results are interesting, but they are a bit out of scope for this paper to include.

Reviewer 2:

Thanks for all the suggestions! We have restructured the paper in the IMRD format and eliminate redundancy in the original sections 1-3. The presentation appears much clearer now.

We included ClinicalBERT and BlueBERT as they are also prominent pretrained language models for the broader biomedical domain. Clinical notes are indeed different from biomedical publications, as you mentioned, and our experiments verify that additional pretraining on them provide little benefit. This is contrary to the prevalent assumption, which expects pretraining on more text (including general domains that are even more different than notes) should help. Our experimental results thus further validate our key observation about domain-specific pretraining.

Thanks to your suggestions, we added Table 8 and Figure 3, as well as more detailed discussion on how the in-domain vocabulary facilitates more efficient learning and error correction in downstream tasks.

As observed by other reviewers, our key contribution is not to propose novel pretraining methods, but instead conduct a systematic and thorough investigation to elucidate the key aspects of domain-specific pretraining and contribute to establishing the best-practice guideline. Entity masking and knowledge-rich pretraining are indeed key research directions. We are very interested in exploring them in future work, but they are a bit out of scope for this paper.

Reviewer 3:

Thanks for the encouraging comments! We indeed aspire to conduct rigorous head-to-head comparison and contribute to best practice for domain-specific pretraining. Also thanks much for all the insightful suggestions! We have incorporated them in the revision, which help improve our paper substantially. 

We conducted additional pretraining experiments as you suggested and added Table 9 with the results. Specifically, we used the PubMed word pieces, pretrained on Wiki/Books, and then pretrained on PubMed. Initially, we shared the expectation that this might perform better than BioBERT using the general-domain vocabulary. Surprisingly, it actually led to slight degradation in performance (second column). To further elucidate the comparison, we conducted another experiment by pretraining from scratch, but only with half of the total compute (third column). Effectively, this is like rerunning your suggested experiment, though without first pretraining on general-domain text. Interestingly, this performs slightly better and attains comparable results as BioBERT. Thanks to your suggestion, these experiments provide more complete head-to-head comparisons with the continual pretraining strategy. 

The second experiment also helps shed light on pretraining time comparison. It uses the same amount of compute as continual pretraining in BioBERT, which builds on top of the standard BERT. The downstream performance is comparable, suggesting that the BERT starting point does not confer much advantage, while imposing the limitation in the vocabulary.

Thanks for the suggestion regarding vocabulary and word piece. In Table 1, we added word pieces for all the biomedical terms. Si et al. (JAMIA-19) is indeed quite relevant. We added it to our reference and discussion on shattering biomedical terms. As Si et al. also observed, word pieces do not necessarily conform with standard morphological analysis from linguistics. They used the general BERT vocabulary, which tends to shatter biomedical terms into many word pieces, as their Supplemental Table 2 shows.

> Table 1: are you claiming that "acetyltransferase" is its own word piece in your vocabulary? I would think not, but that's what the caption implies.  Perhaps show the word pieces here (as suggested above)

Yes. "Aceltylatransferase" is in the PubMed vocabulary. Thanks to your suggestion, we added word pieces for all the biomedical terms in Table 1. The ones with checkmark are included in the corresponding vocabulary. As explained above, BERT vocabulary (BPE or word piece) is not trying to uncover morphological structures, and may include a word if it appears frequent enough in the pretraining corpus.

> Page 13: please provide the timestamp of the PubMed dump

We downloaded the PubMed abstracts and PMC full-text articles in Feb. 2020. We added this to the paper.



==> old-3-model.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BERT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Language Model Pretraining}


In this section, we give a quick overview of neural language model pretraining, using BERT~\cite{devlin2018bert} as a running example.

\subsection{Vocabulary}
\label{subsec:bert-vocab}
We assume that the input consists of text spans, such as sentences separated by special tokens $\tt [SEP]$. To address the problem of out-of-vocabulary words, neural language models generate a vocabulary from subword units, using Byte-Pair Encoding~(BPE)~\cite{sennrich2015bpe} or variants such as WordPiece~\cite{kudo2018sentencepiece}.
Essentially, the BPE algorithm tries to greedily identify a small set of subwords that can compactly form all words in the given corpus. It does this by first shattering all words in the corpus and initializing the vocabulary with characters and delimiters.  It then iteratively augments the vocabulary with a new subword that is most frequent in the corpus and can be formed by concatenating two existing subwords, until the vocabulary reaches the pre-specified size (e.g., 30,000 in standard BERT models or 50,000 in RoBERTa~\cite{liu2019roberta}). In this paper, we use the WordPiece algorithm which is a BPE variant that uses likelihood based on the unigram language model rather than frequency in choosing which subwords to concatenate. 
The text corpus and vocabulary may preserve the case ($\tt cased$) or convert all characters to lower case ($\tt uncased$).

%\hoifung{Hao: Which alg we used, BPE or wordpiece?}
%\chenghao{WordPiece is used. Different from vanilla character-level BPE, WordPiece choose the unit to optimize the training data likelihood.}

\subsection{Model Architecture}
\label{subsec:bert-mdl}
State-of-the-art neural language models are generally based on transformer architectures \cite{vaswani2017attention}, following the recent success of BERT ~\cite{devlin2018bert,liu2019roberta}.
The transformer model introduces a multi-layer, multi-head self-attention mechanism, which has demonstrated superiority in leveraging GPU-based parallel computation and modeling long-range dependencies in texts, compared to recurrent neural networks, such as LSTMs~\cite{hochreiter1997lstm}. 
The input token sequence is first processed by a lexical encoder, which combines a token embedding, a (token) position embedding and a segment embedding (i.e., which text span the token belongs to) by element-wise summation. 
This embedding layer is then passed to multiple layers of transformer modules \cite{vaswani2017attention}. 
In each transformer layer, a contextual representation is generated for each token by summing a non-linear transformation of the representations of all tokens in the prior layer, weighted by the attentions computed using the given token's representation in the prior layer as the query.
The final layer outputs contextual representations for all tokens, which combine information from the whole text span.

%\hoifung{Might be useful to add some illustration of transformer to be self-contained, given that the audience might include less than core ML/NLP folks.}

% \hoifung{Tristan: can u add keyser-ney
% Ney, Hermann; Essen, Ute; Kneser, Reinhard (January 1994). "On structuring probabilistic dependences in stochastic language modeling". Computer Speech & Language. 8 (1): 1–38. doi:10.1006/csla.1994.1001
% }
% %
% \tristan{Yes, added as kneser-ney, updated below}

\subsection{Self-Supervision}
\label{subsec:bert-self-sup}
A key innovation in BERT \cite{devlin2018bert} is the use of a \textbf{Masked Language Model (MLM)} for self-supervised pretraining. 
Traditional language models are typically generative models that predict the next token based on the preceding tokens; for example, n-gram models represent the conditional probability of the next token by a multinomial of the preceding n-gram, with various smoothing strategies to handle rare occurrences~\cite{kneser-ney}. 
Masked Language Model instead randomly replaces a subset of tokens by a special token (e.g., $\tt [MASK]$), and asks the language model to predict them. 
%Essentially, it is a cloze task \cite{taylor1953cloze}, where t
The training objective is the cross-entropy loss between the original tokens and the predicted ones. In BERT and RoBERTa, 15\% of the input tokens are chosen, among which a random 80\% are replaced by $\tt [MASK]$, 10\% are left unchanged and 10\% are randomly replaced by a token from the vocabulary. 
Instead of using a constant masking rate of 15\%, a standard approach is to gradually increase it from 5\% to 25\% with 5\% increment for every 20\% of training epochs, which makes pretraining more stable~\cite{liu2020alum}.  
The original BERT algorithm also uses \textbf{Next Sentence Prediction (NSP)}, which determines for a given sentence pair whether one sentence follows the other in the original text. The utility of NSP has been called into question~\cite{liu2019roberta}, but we include it in our pretraining experiments to enable a head-to-head comparison with prior BERT models.


\subsection{Advanced Pretraining Techniques}
In the original formulation of BERT~\cite{devlin2018bert}, the masked language model (MLM) simply selects random subwords to mask. When a word is only partially masked, it is relatively easy to predict the masked portion given the observed ones. In contrast, whole-word masking (WWM) enforces that the whole word must be masked if one of its subwords is chosen. This has been adopted as the standard approach, as it forces the language model to capture more contextual semantic dependencies. 

In this paper, we also explore adversarial pretraining and its impact on downstream applications. Motivated by successes in countering adversarial attacks in computer vision, adversarial pretraining introduces perturbations in the input embedding layer that maximize the adversarial loss, thus forcing the model to not only optimize the standard training objective (MLM), but also minimize adversarial loss~\cite{liu2020alum}. 
% \tristan{We should say what we do with it, or otherwise indicate that it held value in our current experiments. Putting on my Reviewer 2 hat, this otherwise reads as a throwaway statement to add a citation.}
% \jianfeng{agree that we should summarize our results of adversarial pretraining here.}
% \hoifung{This is a standard BERT section. So I don't want to say too much about the results. Else, we also need to mention positive results for WWM etc. The results are covered in experiments.}
% \tristan{Okay, I'm sold}

%\hoifung{More details to make adv pretraining self-contained?}

%hyperparams

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Domain-Specific LMs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Biomedical Language Model Pretraining}
\label{sec:domain}

%\hoifung{Use mixed-domain pretraining instead of continual pretraining?}

Pretraining language models using general text has proven beneficial for applications in open domains, such as newswire and the Web~\cite{devlin2018bert,liu2019roberta}. However, there are also many high-value applications in specialized domains, many of which have an abundance of in-domain text, such as biomedicine, finance, and legal. In this paper, we will use biomedicine as a running example in our study of domain-specific pretraining. In other words, biomedical text is considered in-domain, while others are regarded as out-domain.

Intuitively, using in-domain text in pretraining should help with domain-specific applications. Indeed, prior work has shown that pretraining with PubMed text leads to better performance in biomedical NLP tasks \cite{lee2019bioberts,beltagy2019scibert,peng2019transfer}. 
The main question is whether pretraining should include text from other domains. 
The prevailing assumption is that pretraining can always benefit from more text, including out-domain text. And, in fact, none of the prior biomedical-related BERT models have been pretrained using purely biomedical text \cite{lee2019bioberts,beltagy2019scibert,peng2019transfer}. 
In this paper, we challenge this assumption and show that {\em domain-specific pretraining from scratch} is superior to {\em mixed-domain pretraining} for downstream applications.


\subsection{Mixed-Domain Pretraining}

%\hoifung{Should we include ClinicalBERT?}
%\tristan{Yes, for reference there are 3 ClinicalBERT: 
%1) Us (ClinicalNLP): https://arxiv.org/abs/1904.03323  
%2) Rajesh (CHIL): https://arxiv.org/abs/1904.05342
%3) Kirk (JAMIA): https://arxiv.org/abs/1902.08691}

% \hoifung{Tristan: can u add a MIMIC ref below?}

The standard approach to pretraining a biomedical BERT model conducts {\em continual pretraining} of a general-domain pretrained model, as exemplified by BioBERT~\cite{lee2019bioberts}. 
Specifically, this approach would initialize with the standard BERT model~\cite{devlin2018bert}, pretrained using Wikipedia and BookCorpus. It then continues the pretraining process with MLM and NSP using biomedical text. 
In the case of BioBERT, continual pretraining is conducted using PubMed abstracts and full text. BlueBERT~\cite{peng2019transfer} uses both PubMed text and de-identified clinical notes from MIMIC-III~\cite{mimic}. 

Note that in the continual pretraining approach, the vocabulary is the same as the original BERT model, in this case the one generated from Wikipedia and BookCorpus. While convenient, this is a major disadvantage for this approach, as the vocabulary is not representative of the target biomedical domain.

Compared to the other biomedical-related pretraining efforts, SciBERT~\cite{beltagy2019scibert} is a notable exception as it generates the vocabulary and pretrains from scratch, using biomedicine and computer science as representatives for the scientific literature. However, from the perspective of biomedical applications, SciBERT still adopts the mixed-domain pretraining approach, as computer science text is clearly out-domain.

%\jianfeng{Does SciBERT outperform BioBERT? Is the biomedical text used for SciBERT the same as what we use for domain-specific pre-training? Also need to clarify how we decide a text is in-domain or out-domain. For example, if we define a scientific paper domain, both biomedical and compute science texts are in-domain. This depends on end applications.}
%\hoifung{Good pt. Added in-dom vs out-domain at the top of sec. Also fixed SciBERT. SciBERT underperforms BioBERT.}


\subsection{Domain-Specific Pretraining from Scratch}

The mixed-domain pretraining approach makes sense if the target application domain has little text of its own, and can thereby benefit from pretraining using related domains. 
However, this is not the case for biomedicine, which has over thirty million papers in PubMed, and adds over a million each year. 
{\em We thus hypothesize that domain-specific pretraining from scratch is a better strategy for biomedical language model pretraining.}

\begin{table}[h]
    \centering
\begin{tabular}{llccc}
%\toprule
\specialrule{1pt}{1.5pt}{1.5pt}

              Biomedical Term &  Category & BERT & SciBERT & PubMedBERT (Ours) \\
\midrule
          diabetes &   disease &    \checkmark &       \checkmark &    \checkmark \\
          leukemia &   disease &    \checkmark &       \checkmark &    \checkmark \\
           lithium &  drug &    \checkmark &       \checkmark &    \checkmark \\
           insulin &      drug &    \checkmark &       \checkmark &    \checkmark \\
               DNA &      gene &    \checkmark &       \checkmark &    \checkmark \\
          promoter &      gene &    \checkmark &       \checkmark &    \checkmark \\
      hypertension &   disease &      &       \checkmark &    \checkmark \\
       nephropathy &   disease &      &       \checkmark &    \checkmark \\
          lymphoma &   disease &      &       \checkmark &    \checkmark \\
         lidocaine &  drug &      &       \checkmark &    \checkmark \\
     oropharyngeal &   organ &      &         &    \checkmark \\
     cardiomyocyte &   cell &      &         &    \checkmark \\
   chloramphenicol &      drug &      &         &    \checkmark \\
              RecA &      gene &      &         &    \checkmark \\
 acetyltransferase &      gene &      &         &    \checkmark \\
         clonidine &  drug &      &         &    \checkmark \\
          naloxone &  drug &      &         &    \checkmark \\
\bottomrule
\end{tabular}
    \caption{Comparison of common biomedical terms in vocabularies used by the standard BERT, SciBERT and PubMedBERT (ours). A~$\checkmark$~indicates the biomedical term appears in the corresponding vocabulary, otherwise the term will be shattered into small subwords.}
    \label{tab:vocab_comparison}
\end{table}

A major advantage of domain-specific pretraining from scratch stems from having an in-domain vocabulary. 
\autoref{tab:vocab_comparison} compares the vocabularies used in various pretraining strategies. BERT models using continual pretraining are stuck with the original vocabulary from the general-domain corpora, which does not contain many common biomedical terms. 
Even for SciBERT, which generates its vocabulary partially from biomedical text, the deficiency compared to a purely biomedical vocabulary is substantial.
As a result, standard BERT models are forced to divert parametrization capacity and training bandwidth to model biomedical terms using fragmented subwords. 
% For example, \texttt{lymphoma}, a common medical term, is divided into four pieces ($[$\texttt{l, \#\#ym, \#\#ph, \#\#oma}$]$) by BERT, and \texttt{acetyltransferase} is shattered into seven ($[$\texttt{ace, \#\#ty, \#\#lt, \#\#ran, \#\#sf, \#\#eras, \#\#e}$]$).
For example, naloxone, a common medical term, is divided into four pieces ([na, ##lo, ##xon, ##e]) by BERT, and acetyltransferase is shattered into seven pieces ([ace, ##ty, ##lt, ##ran, ##sf, ##eras, ##e]) by BERT. Both terms appear in the vocabulary of PubMedBERT.
% UPDATED EXAMPLES FOR PR PUSH
% Option #1:
%     For example, lymphoma, a common medical term, is divided into four pieces ([l, ##ym, ##ph, ##oma]) by BERT but present in the vocabularies of SciBERT and PubMedBERT; similarly, acetyltransferase is shattered into seven pieces ([ace, ##ty, ##lt, ##ran, ##sf, ##eras, ##e]) by BERT and two pieces ([acetyl, ##transferase]) by SciBERT but present in the vocabulary of PubMedBERT.
%
% Option #2:
% For example, naloxone, a common medical term, is divided into four pieces ([na, ##lo, ##xon, ##e]) by BERT and three pieces ([nal, ##oxo, ##ne]) by SciBERT; similarly, acetyltransferase is shattered into seven pieces ([ace, ##ty, ##lt, ##ran, ##sf, ##eras, ##e]) by BERT and two pieces ([acetyl, ##transferase]) by SciBERT. Both terms appear in the vocabulary of PubMedBERT.
%
%\hoifung{Hao: Insert some ridiculously fragmented examples}
% \tristan{Which did these come from?}
% \hoifung{From BERT, I assume. I didn't elaborate for SciBERT.}
% \tristan{Confirmed these are from BERT and that SciBERT tokenizaiton is better}

Another advantage of domain-specific pretraining from scratch is that the language model is trained using purely in-domain data. 
% No model capacity is wasted on out-domain linguistic phenomena. 
For example, SciBERT pretraining has to balance optimizing for biomedical text and computer science text, the latter of which is unlikely to be beneficial for biomedical applications. 
Continual pretraining, on the other hand, may potentially recover from out-domain modeling, though not completely. Aside from the vocabulary issue mentioned earlier, neural network training uses non-convex optimization, which means that continual pretraining may not be able to completely undo suboptimal initialization from the general-domain language model. 
% Of course, the initialization may also be beneficial if it captures common linguistic regularities that transcend the domains, so the effect could be mixed.

In our experiments, we show that domain-specific pretraining with in-domain vocabulary confers clear advantages over mixed-domain pretraining, be it continual pretraining of general-domain language models, or pretraining on mixed-domain text.

%both in-domain vocabulary and pretraining from scratch confer clear advantages. In fact, even with the out-domain vocabulary, pretraining from purely biomedical text still leads to better performance in downstream NLP tasks compared to continual pretraining, thus confirming that on balance, inclusion of out-domain text in biomedical pretraining is a net loss.
%\hoifung{Double check w. Hao}
%\chenghao{For all our bert models with BERT vocab, they are trained in the continual pretraining fashion (mixed-domain pretraining, i.e. initialized from BERT model and continual training). In our preliminary study, we found that pretraining from scratch with BERT-vocab is not as effective as with Pubmed-vocab. We didn't do anything with BERT-vocab from scratch afterwards.}

%training time?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BLURB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{BLURB: A Comprehensive Benchmark for Biomedical NLP}

\begin{table}[ht]
\begin{center}
\begin{tabular}{lcccc}
\specialrule{1pt}{1.5pt}{1.5pt}
&  BioBERT~\cite{lee2019bioberts} &  SciBERT~\cite{beltagy2019scibert} &  BLUE~\cite{peng2019transfer} &  BLURB \\
\midrule
BC5-chem~\cite{li2016biocreative}     &  \checkmark &  \checkmark &  \checkmark & \checkmark  \\
BC5-disease~\cite{li2016biocreative}     &  \checkmark &  \checkmark &  \checkmark & \checkmark  \\
NCBI-disease~\cite{dougan2014ncbi}     &  \checkmark &  \checkmark &  - & \checkmark  \\
BC2GM~\cite{smith2008overview}     &  \checkmark & - &  - & \checkmark  \\
JNLPBA~\cite{collier-kim-2004-introduction}     &  \checkmark &  - &  - & \checkmark  \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
EBM PICO~\cite{nye2018corpus}     &  - &  \checkmark &  - & \checkmark  \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
ChemProt~\cite{krallinger2017overview}     &  \checkmark &  \checkmark &  \checkmark & \checkmark  \\
DDI~\cite{herrero2013ddi}     &  \checkmark &  - &  \checkmark & \checkmark  \\
GAD~\cite{bravo2015extraction}     &  \checkmark &  - &  - & \checkmark  \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
BIOSSES~\cite{souganciouglu2017biosses}     &  - &  - &  \checkmark & \checkmark  \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
HoC~\cite{hanahan2000hallmarks}     &  - &  - & \checkmark & \checkmark  \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
PubMedQA~\cite{jin2019PubMedqa}     & -  &  - &  - & \checkmark  \\
BioASQ~\cite{nentidis2019results}     &  \checkmark &  - &  - & \checkmark  \\
\specialrule{1pt}{1.5pt}{1.5pt}
\end{tabular}
\end{center}
\caption{Comparison of the biomedical datasets in prior language model pretraining studies and BLURB. \label{tab:paper-dataset}}
\end{table}
% \tristan{Would be nice to have citations in the table in place of paper currently. I.e., it would read BioBERT [number]. As a reference, anyone then looking just at the table gets more information that they might be looking for.}
% \hoifung{Agree! Let's do it. You can find all in Sec 4.}
% \tristan{Done, though it might be nice to include a hidden column to improve the spacing for the citations}.

%\hoifung{Rob: please insert task stat table} 
%\aiden{Added stats table with train/dev/test size and standard metrics we suggest using. }
%\hoifung{TODO: Add stats for the two NER tasks; fix JNLPBA}
%\hoifung{Aiden: Why is PICO macro F1? Why are rel micro F1? (What's macro there?)}
%\aiden{Micro F1 is the standard metric across several papers.Macro f1 is the arithmetic mean of P,I, and O classes.}

%\hoifung{Explain macro; move pico to NER}
%\hoifung{Explain why BLUE is not sufficient; why pure biomed; fix all stat}

The ultimate goal of language model pretraining is to improve performance on a wide range of downstream applications. 
In general-domain NLP, the creation of comprehensive benchmarks, such as GLUE~\cite{wang19iclr_glue,wang2019superglue}, greatly accelerates advances in language model pretraining by enabling head-to-head comparisons among pretrained language models. % and have become the gold standard for evaluation. %GLUE \cite{glue} is the most prominent example, which inspires the creation of other benchmarks such as SuperGLUE, X-GLUE, {\bf anything else?}.
In contrast, prior work on biomedical pretraining tends to use different tasks and datasets for downstream evaluation, as shown in \autoref{tab:paper-dataset}. This makes it hard to assess the impact of pretrained language models on the downstream tasks we care about. 
To the best of our knowledge, BLUE~\cite{peng2019transfer} is the first attempt to create an NLP benchmark in the biomedical domain. We aim to improve on its design by addressing some of its limitations. 
First, BLUE has limited coverage of biomedical applications used in other recent work on biomedical language models, as shown in \autoref{tab:paper-dataset}. For example, it does not include any question-answering task. More importantly, BLUE mixes PubMed-based biomedical applications (six datasets such as BC5, ChemProt, and HoC) with MIMIC-based clinical applications (four datasets such as i2b2 and MedNLI). Clinical notes differ substantially from biomedical literature, to the extent that we observe BERT models pretrained on clinical notes perform poorly on biomedical tasks, similar to the standard BERT. Consequently, it is advantageous to create separate benchmarks for these two domains.

To facilitate investigations of biomedical language model pretraining and help accelerate progress in biomedical NLP, we create a new benchmark, the {\em Biomedical Language Understanding \& Reasoning Benchmark (BLURB)}. 
We focus on PubMed-based biomedical applications, and leave the exploration of the clinical domain, and other high-value verticals to future work. 
%biomedical literature and related applications, and leave the creation of a clinical benchmark to future work. 
To make our effort tractable and facilitate head-to-head comparison with prior work, we prioritize the selection of datasets used in recent work on biomedical language models, and will explore the addition of other datasets in future work. 

%Peng et al. 2019 
%By creating BLURB, we hope to fill in this gap and facilitate systematic comparison of language model pretraining for biomedical NLP. As we can see above, the results clearly elucidate the impact of domain-specific pretraining compared to mixed-domain pretraining.
%To stay true to our goal to study domain-specific pretraining, we limit the scope of the benchmark to biomedical NLP tasks, specifically ones with input text from PubMed articles. We leave the exploration of clinical domains (i.e., input text from clinical notes) or other high-value verticals to future work.

\begin{table}[ht]
\begin{center}
\begin{tabular}{llllll}
%\toprule
\specialrule{1pt}{1.5pt}{1.5pt}

Dataset  &  Task & Train & Dev & Test & Evaluation Metrics \\
\midrule
%\specialrule{1pt}{1.5pt}{1.5pt}
%\specialrule{0.05pt}{1.5pt}{1.5pt}
BC5-chem    &       NER &    5203 &         5347 &       5385 &        F1 entity-level \\
BC5-disease &       NER&    4182 &         4244 &       4424 &         F1 entity-level \\
NCBI-disease      &       NER&    5134 &     787     &     960   &          F1 entity-level \\
BC2GM      &       NER&     15197&         3061 &     6325   &          F1 entity-level \\
JNLPBA      &       NER&    46750&       4551   &    8662    &          F1 entity-level \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
EBM PICO &       PICO&   339167 &         85321 &   16364     &         Macro F1 word-level \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
ChemProt    &       Relation Extraction&    18035 &         11268 &       15745 &         Micro F1 \\
DDI         &       Relation Extraction&    22233 &         5559 &       5716 &        Micro F1 \\
GAD         &       Relation Extraction&    4261 &        534 &        535 &         Micro F1 \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
BIOSSES     &       Sentence Similarity&    64&             16&       20 &         Pearson \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
HoC         &       Document Classification&    1295 &         186 &       371 &         Average Micro F1 \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
PubMedQA    &       Question Answering& 450 &         50 &       500 &         Accuracy \\
BioASQ      &       Question Answering& 670 &         75 &       140 &         Accuracy \\
\bottomrule
\end{tabular}
\end{center}
\caption{Datasets used in the BLURB biomedical NLP benchmark. We list the numbers of instances in train, dev, and test (e.g., entity mentions in NER and PICO elements in evidence-based medical information extraction).
%We list here the No. entities for NER and PICO tasks, and No. Sentences for all other tasks.
\label{tab:task-stats}
}
\end{table}
%\hoifung{Aiden/Rob: "sentences for other tasks" - what about HoC, QA? Also, DDI not strictly per-sentence, right? Do you mean instances for all tasks? }
%\aiden{Yes, instance is more accurate.}

BLURB is comprised of a comprehensive set of biomedical NLP tasks from publicly available datasets, including named entity recognition (NER), %population, intervention, control and outcomes 
evidence-based medical information extraction (PICO), relation extraction, sentence similarity, document classification, and question answering. 
%To make our effort tractable, we prioritize datasets featured in recent language model evaluations involving the biomedical domain. 
See \autoref{tab:task-stats} for an overview of the BLURB datasets. 
%Our selection spans a wide range of task complexity and supervision regimes. 
For question answering, prior work has considered both classification tasks (e.g., whether a reference text contains the answer to a given question) and more complex tasks such as list and summary \cite{nentidis2019results}. The latter types often require additional engineering effort that are not relevant to evaluating neural language models. For simplicity, we focus on the classification tasks such as yes/no question-answering in BLURB, and leave the inclusion of more complex question-answering to future work.

To compute a summary score for BLURB, the simplest way is to report the average score among all tasks. However, this may place undue emphasis on simpler tasks such as NER for which there are many existing datasets. Therefore, we group the datasets by their task types, compute the average score for each task type, and report the macro average among the task types. 
To help accelerate research in biomedical NLP, we release the BLURB benchmark as well as a leaderboard at {\url{http://aka.ms/BLURB}}.

Below are detailed descriptions for each task and its corresponding dataset.

%%%%%%%%%%%%%%%%%%%%%%%
\eat{
\hoifung{
BC5: abstracts or full text?

BC2: what's ALTGENE? double-check sentence 20K? We didn't use unreleased test, right? 

JNLPBA: confirm we didn't use crichton data but follow their split
}
\aiden{
BC5: is abstracts.

BC2: ALTGENE mean alternative gene: alternate boundaries that are judged by human annotators to be essentially equivalent references. There are in total 20k sentences, and a standard train/test split. We use a prepossessed version which split 2500 sentences from train as the dev data. train/dev/test: 12500, 2500, 5000 #sentences

JNLPBA: Ye, we only follow their dev split since there is official standard train/test split.
}
}
%%%%%%%%%%%%%%%%%%%%%%%%

%\hoifung{BC2: so total is 20K, dev is 2500, what is train/test number?}

\subsection{Named Entity Recognition (NER)}
\paragraph{BC5-Chemical \& BC5-Disease} The BioCreative V Chemical-Disease Relation corpus \cite{li2016biocreative} was created for evaluating relation extraction of drug-disease interactions, but is frequently used as a NER corpus for detecting chemical (drug) and disease entities. The dataset consists of 1500 PubMed abstracts broken into three even splits for training, development, and test. We use a pre-processed version of this dataset generated by \citet{crichton2017neural}, discard the relation labels, and train NER models for chemical (\textit{BC5-Chemical}) and disease (\textit{BC5-Disease}) separately.

\paragraph{NCBI-Disease} The Natural Center for Biotechnology Information Disease corpus \cite{dougan2014ncbi} contains 793 PubMed abstracts with 6892 annotated disease mentions linked to 790 distinct disease entities. We use a pre-processed set of train, development, test splits generated by \citet{crichton2017neural}.

\paragraph{BC2GM} The Biocreative II Gene Mention corpus \cite{smith2008overview} consists of sentences from Pubmed abstracts with manually labeled gene and alternative gene entities. Following prior work, we focus on the gene entity annotation. In its original form, BC2GM contains 15000 train and 5000 test sentences. %while 5000 unreleased evaluation sentences were used to evaluate entries to the BC2GM workshop. 
We use a pre-processed version of the dataset generated by \citet{crichton2017neural}, which carves out 2500 sentences from the training data for development.

\paragraph{JNLPBA} The Joint Workshop on Natural Language Processing in Biomedicine and its Applications shared task \cite{collier-kim-2004-introduction} is a NER corpus on PubMed abstracts. The entity types are chosen for molecular biology applications: protein, DNA, RNA, cell line, and cell type. 
Some of the entity type distinctions are not very meaningful. For example, a gene mention often refers to both the DNA and gene products such as the RNA and protein. 
Following prior work that evaluates on this dataset \cite{lee2019bioberts}, we ignore the type distinction and focus on detecting the entity mentions. 
We use the same train, development, and test splits as in \citet{crichton2017neural}.
%We use a pre-processed version of JNLPBA and the train, development, and test splits generated by \cite{crichton2017neural}.

%\aiden{JNLPBA: We processed the data from the official corpus. We discarded the entity types to make it the same as other NER tasks with only one entity type. We made the train/dev split the same as in [7]. }

\subsection{Evidence-Based Medical Information Extraction (PICO)}

\paragraph{EBM PICO} The Evidence-Based Medicine corpus \cite{nye2018corpus} contains PubMed abstracts on clinical trials, where each abstract is annotated with P, I, and O in PICO: Participants (e.g., \texttt{diabetic patients}), Intervention (e.g., \texttt{insulin}), Comparator (e.g., \texttt{placebo}) and Outcome (e.g., \texttt{blood glucose levels}). Comparator (C) labels are omitted as they are standard in clinical trials: placebo for passive control and standard of care for active control. There are 4300, 500, and 200 abstracts in training, development, and test, respectively.
% \jianfeng{Out of curiosity, why does PICO data only contain P, I, O labels, not C?}
% \hoifung{C is pretty standard - you just compare a trial arm w. a control arm (placebo for passive control and standard care for active control).}
% \tristan{I think the comment here is why is the *C* missing from the list above? --- Answer is that the task online contains PIO labels.}
% \hoifung{Yes - I tried to explain why they skip C: there is no point as it's standard.}
%These abstracts were annotated with PICO entities, which are named entity types specifically relevant to biomedical and clinical research: Populations (e.g., diabetics), Interventions (insulin), Comparators (placebo) and Outcomes (blood glucose levels). 
The training and development sets were labeled by Amazon Mechanical Turkers, whereas the test set was labeled by Upwork contributors with prior medical training. EBM PICO provides labels at the word level for each PIO element. For each of the PIO elements in an abstract, we tally the F1 score at the word level, and then compute the final score as the average among PIO elements in the dataset. Occasionally, two PICO elements might overlap with each other (e.g., a participant span might contain within it an intervention span). In EBM-PICO, about 3\% of the PIO words are in the overlap. Note that the dataset released along with SciBERT appears to remove the overlapping words from the larger span (e.g., the participant span as mentioned above). We instead use the original dataset~\cite{nye2018corpus} and their scripts for preprocessing and evaluation.

%\hoifung{No C, participant}
%\aiden{3 elements: participants, interventions, outcomes.}
%, but does not provide start or end locations for multi-word entities or distinguish between adjacent words belonging to the same entity or multiple-word entities, so we calculate word-level performance for this dataset.
%\aiden{Labels for each P/I/O element are separated since they occasionally overlap (for 0.03 of tokens). To combine them for joint learning, we followed the official example script. We made our own train/dev split.}
%\hoifung{What does it mean by official example / own train/dev split? macro F1 per element or per abs?}
%\aiden{F1 per element}
%\hoifung{Michael: What's the train/dev numbers of abstracts?} (completed  -michael)

%\michael{team: These examples were copied directly from EBM PICO. I think these examples are great, but am not sure if we should come up with new ones.}
%rob{I personally think these are great examples, it is more concise than most of the examples in EBM PICO!}

\subsection{Relation Extraction}
\paragraph{ChemProt} The Chemical Protein Interaction corpus \cite{krallinger2017overview} consists of PubMed abstracts annotated with chemical-protein interactions between chemical and protein entities. There are 23 interactions organized in a hierarchy, with 10 high-level interactions (including $\tt NONE$). 
The vast majority of relation instances in ChemProt are within single sentences. Following prior work \cite{lee2019bioberts,beltagy2019scibert}, we only consider sentence-level instances.
%each of which may have zero or more sub-interactions. 
%We follow the ChemProt authors' suggestions and focus on classifying each entity pair as belonging to one of five high-level interactions or not (CPR:3, CPR:4, CPR:5, CPR:6, CPR:9, and "$\tt false$"). 
We follow the ChemProt authors' suggestions and focus on classifying five high-level interactions --- $\tt UPREGULATOR~~(CPR:3)$, $\tt DOWNREGULATOR~~ (CPR:4)$, $\tt AGONIST~~ (CPR:5)$, $\tt ANTAGONIST~~ (CPR:6)$, $\tt SUBSTRATE ~~(CPR:9)$ --- as well as everything else ($\tt false$).
The ChemProt annotation is not exhaustive for all chemical-protein pairs.
Following previous work~\cite{peng2019transfer,lee2019bioberts}, we expand the training and development sets by assigning a $\tt false$ label for all chemical-protein pairs that occur in a training or development sentence, but do not have an explicit label in the ChemProt corpus. 
Note that prior work uses slightly different label expansion of the test data. To facilitate head-to-head comparison, we will provide instructions for reproducing the test set in BLURB from the original dataset.

%\hoifung{So when we evaluate, did we include the expanded labels?}
%\aiden{Yes we do include expanded labels, as done by other papers.}
%We increase the maximum sequence length from the standard 128 to 256 tokens to capture the full sequence in 99\% of all cases.
%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{
\aiden{
All CPR(chemprot relations) were grouped into 10 semantically related classes that share underlying biological properties. 
Mapping of CPR to actual relations
CPR:1	PART_OF
CPR:2	REGULATOR|DIRECT_REGULATOR|INDIRECT_REGULATOR
CPR:3	UPREGULATOR|ACTIVATOR|INDIRECT_UPREGULATOR
CPR:4	DOWNREGULATOR|INHIBITOR|INDIRECT_DOWNREGULATOR
CPR:5	AGONIST|AGONIST-ACTIVATOR|AGONIST-INHIBITOR
CPR:6	ANTAGONIST
CPR:7	MODULATOR|MODULATOR-ACTIVATOR|MODULATOR-INHIBITOR
CPR:8	COFACTOR
CPR:9	SUBSTRATE|PRODUCT_OF|SUBSTRATE_PRODUCT_OF
CPR:10	NOT
}}
%%%%%%%%%%%%%%%%%%%%%%%%%

%\aiden{chemprot:We also expand test data this way(adding false cases). It's not fair comparison considering each of the three papers have its own version of test data. However, we are the only one who provides the script for data preprocessing from official data.}

%\hoifung{How did other produce negative for test? False = no interaction? What's each of the CPR meaning? Why those five? An instance could be none for all five, right?}

%\hoifung{DDI: can instances cross sent?}
%\aiden{DDI: Unlike chrmprot, instances in DDI are all within sent. }

\paragraph{DDI} The Drug-Drug Interaction corpus \cite{herrero2013ddi} was created to facilitate research on pharmaceutical information extraction, with a particular focus on pharmacovigilance. It contains sentence-level annotation of drug-drug interactions on PubMed abstracts.
%The corpus consists of 233 Medline abstracts and 792 Drugbank texts with annotations consisting of 18502 pharmaceutical substances and 5028 drug-drug interactions. 
%The original dataset was split into 714 files for training and 191 for test. 
Note that some prior work \cite{peng2019transfer,zhang2018drug} discarded 90 training files that the authors considered not conducive to learning drug-drug interactions. We instead use the original dataset and produce our train/dev/test split of 624/90/191 files.
%\cite{?} found that 90 training files are not relevant for drug-drug interaction. Like \cite{BLUE}, we filter these files.

%\hoifung{The counts don't add up. Are 90 in 714?}
%\aiden{We didn't follow the filtering. DDI corpus has extra test data for DDI NER task so the number don't add up.  } 
%\hoifung{Can you fill in the number of train/dev/test above?}

% \hoifung{Tristan: can you add citation: zhang2018ddi https://academic.oup.com/bioinformatics/article/34/5/828/4565590}

%We generated our own train, test, and development splits which we make available at http://aka.ms/BLURB. Similarily to ChemProt a maximum sequence length of 256 tokens is used to handle the long input sequences.
%\aiden{DDI:We made our own train/dev split. We use all 714 train files and 191 test files from the original corpus. https://academic.oup.com/bioinformatics/article/34/5/828/4565590 this work claimed 90 train files to have no relevance to "DDI" and removed them. BLUE didn't cite this work but used their filtered dataset. I didn't follow this filtering but used the original set.}

%\michael{Is using http://aka.ms/BLURB here the right approach?}
%\michael{team: Details? Do we need to make these splits available for download on the site?} 
%\rob{I think we can create the splits in preprocessing script for the data so need to have this information on the download site}.
%\aiden{To be specific, there is official DDI test data and we applied train/dev split.}

\paragraph{GAD} The Genetic Association Database corpus  \cite{bravo2015extraction} was created semi-automatically using the Genetic Association Archive.\footnote{\url{http://geneticassociationdb.nih.gov/}} Specifically, the archive contains a list of gene-disease associations, with the corresponding sentences in the PubMed abstracts reporting the association studies. Bravo et al.~\cite{bravo2015extraction} used a biomedical NER tool to identify gene and disease mentions, and create the positive examples from the annotated sentences in the archive, and negative examples from gene-disease co-occurrences that were not annotated in the archive. We use an existing preprocessed version of GAD and its corresponding train/dev/test split created by \citet{lee2019bioberts}.

%\hoifung{Is it sentences based? Any stats about num sentences/abstracts? Is it gene-disease?}

%\hoifung{BIOSSES: that each sentence must cite at least one other article??}

\subsection{Sentence Similarity}
\paragraph{BIOSSES} The Sentence Similarity Estimation System for the Biomedical Domain \cite{souganciouglu2017biosses} contains 100 pairs of PubMed sentences each of which is annotated by five expert-level annotators with an estimated similarity score in the range from 0 (no relation) to 4 (equivalent meanings). It is a regression task, with the average score as the final annotation.
We use the same train/dev/test split in \citet{peng2019transfer} and use Pearson correlation for evaluation.

%\hoifung{Annotator biomed background or turker? Would score be continuous number? What's the loss function?}
%\aiden{The only mention about the background of annotators is "human experts". Their score is discrete as 0,1,2,3,4. The objective function is MSE and the evaluation metric is Pearson. }
%The sentence pairs $(s_1, s_2)$ are labeled with an estimated similarity score in the range from 0 (no relation) to 4 (equivalent meanings). We use a preprocessed version of the BIOSSES corpus with fixed train, test, and development sets generated by \cite{peng2019transfer} and format the input to BERT models as \texttt{[CLS]} $s_1$ \texttt{[SEP]} $s_2$.
%\aiden{BIOSSES: Sentence pairs are labelled by 5 annotators. We use the average score as the final label. We processed the data from official data and adopted a existed version of train/dev/test split.}
 
\subsection{Document Classification}

%\hoifung{Actually, those 272 are NONE label (no hallmark) and should be included (all false). Should we redo exps?}

\paragraph{HoC} The Hallmarks of Cancer corpus was motivated by the pioneering work on cancer hallmarks \cite{hanahan2000hallmarks}. It contains annotation on PubMed abstracts with binary labels each of which signifies the discussion of a specific cancer hallmark. The authors use 37 fine-grained hallmarks which are grouped into ten top-level ones. We focus on predicting the top-level labels.
The dataset was released with 1499 PubMed abstracts \cite{baker2015automatic} and has since been expanded to 1852 abstracts \cite{baker2017cancer}. Note that \citet{peng2019transfer} discarded a control subset of 272 abstracts that do not discuss any cancer hallmark (i.e., all binary labels are false). They also used a different evaluation metric. We instead adopt the original dataset and its evaluation metric (average micro F1 across the ten cancer hallmarks), and create the train/dev/test split, as they are not available previously.\footnote{The original authors used cross-validation for their evaluation.}

%\hoifung{Did the original authors provide any split?}

%as a hierarchical labeling scheme to label every sentence with a total of 37 binary labels. These labels are composed of 10 top-level binary labels, each of which contains one to 5 binary sublabels. Our experiments do not incorporate knowledge of the label hierarchy and jointly predict all 10 labels as individual sigmoidal outputs. Here we follow the data processing approach of \cite{peng2019transfer} and created matching train/dev/test splits.
%We prepend input sentences with the \texttt{[CLS]} token and truncate inputs to 128 tokens. %HoC uses the Hallmarks of Cancer \cite{hanahan2000hallmarks} as a hierarchical labeling scheme to label every sentence with a total of 37 binary labels. These labels are composed of 10 top-level binary labels, each of which contains one to 5 binary sublabels. Our experiments do not incorporate knowledge of the label hierarchy and jointly predict all 10 labels as individual sigmoidal outputs. Here we follow the data processing approach of \cite{peng2019transfer} and created matching train/dev/test splits.
%\aiden{HoC: 1852 docs in the corpus while 272 has no label. We follow a prior work and use the remaining 1580. No official split provided, we made our own version of train/dev/test split of 7:1:2.}
%\rob{Updated this to say we follow the processing of BLUE}
%\michael{team: HoC's author requests that these 4 papers are cited: baker2015automatic (the original HoC paper), baker2017cancer (annotation tool), baker2016cancer (CNN-based approach), and baker2017initializing (hierarchical approach).}



\subsection{Question Answering (QA)}

\paragraph{PubMedQA} The PubMedQA dataset \cite{jin2019PubMedqa} contains a set of research questions, each with a reference text from a PubMed abstract as well as an annotated label of whether the text contains the answer to the research question (yes/maybe/no). We use the original train/dev/test split with 450, 50, and 500 questions, respectively.
%The PubMedQA dataset \cite{jin2019PubMedqa} consists of biomedical and yes/maybe/no questions with train, dev, and test splits that contain 450, 50, and 500 questions, respectively. We limit our experiments to the yes/no/maybe questions. Each training example is composed of a question $q$, a short reference text $R$ from a PubMed abstract that may contain the answer to the question, and a yes/no/maybe answer label $a$. In our experiments, we generate a 3-output softmax prediction over the yes, no, and maybe labels. Similar to our treatment of BioASQ, we use a BERT input representation of \texttt{[CLS]q[SEP]R} and truncate the input length to 512 tokens.

\paragraph{BioASQ} The BioASQ corpus \cite{nentidis2019results} contains multiple question answering tasks annotated by biomedical experts, including yes/no, factoid, list, and summary questions. 
Pertaining to our objective of comparing neural language models, we focus on the the yes/no questions (Task 7b), and leave the inclusion of other tasks to future work. Each question is paired with a reference text containing multiple sentences from a PubMed abstract and a yes/no answer. 
We use the official train/dev/test split of 670/75/140 questions.

% \hoifung{Fill in train/dev/test split above.}


%The BioASQ Task 7b corpus \cite{nentidis2019results} consists of multiple question answering tasks manually annotated by biomedical experts. It consists of yes/no, factoid, list, and summary questions, but we limit our experiments to the yes/no questions. Each question $q$ is paired with reference text $R$ containing multiple sentences from a PubMed abstract and a yes/no answer $a$. BioASQ's reference text is often very long, so we use a BERT input representation of \texttt{[CLS]q[SEP]R} and truncate the input length to 512 tokens. Predictions are made using a sigmoidal output in the range 0 (for "no") to 1 (for "yes").

%We also considered an alternative input representation for BioASQ that avoids truncating the reference text. In this experiment, we split the reference text $R$ into sentences $r_i$  and trained over tuples \texttt{(q, r\_i, a)} as separate training examples. During inference, we used the max of the individual sentence predictions as the final prediction for a given question with the interpretation that we expect the answer to these questions be "no" unless we see evidence that the answer is "yes" in one or more sentences. We found that this approach did not perform well and include its description here for posterity.



==> old-32-model-fine-tune.tex <==
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Fine-Tuning
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Task-Specific Fine-Tuning}
\label{sec:fine-tuning}

\begin{figure}
    \centering

%    \includegraphics[width=0.9\textwidth]{figs/fine-tuning.pdf}
	 \adjustbox{trim={0.1\width} {0.1\height} {0.1\width} {0.05\height},clip}{
     \includegraphics[width=1.0\textwidth]{figs/re-ft.pdf}
     }
    \caption{A general architecture for task-specific fine-tuning of neural language models, with a relation-extraction example. Note that the input goes through additional processing such as word-piece tokenization in the neural language model module.
    %The upper part is the typical continual pretraining paradigm replying on a vocabulary and a generic language model (BERT) based on general domain text source, such as Wikipedia, children books and web text. The lower part illustrates the domain-specific pretraining from scratch with a domain specific vocabulary.
    }
    \label{fig:fine-tuning}
\end{figure}


%%%%%%%%%%%%%%%%%%%
\eat{
\begin{table}[h]
    \centering
\begin{tabular}{lll}
\toprule
            Task                    &  Problem Formulation        &  Epoch Range      \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
            NER                         & Token Classification  & 20 - 60 \\
            PICO                        & Token Classification  & 2 - 3    \\
            Relation Extraction         & Sequence Classification   & 5 - 20 \\
            Sentence Similarity         & Sequence Regression       & 40 - 60 \\
            Document Classification     & Sequence Classification   & 10 - 30 \\
            Question Answering          & Sequence Classification   & 10 - 20 \\
\bottomrule
\end{tabular}
    \caption{Standard problem formulation}
    \label{tab:task_model_choices}
\end{table}

\begin{table}[h]
    \centering
\begin{tabular}{llll}
\toprule
                 Model &         Components          &  Standard     &   Variants \\
\specialrule{0.05pt}{1.5pt}{1.5pt}
            Sequence Classification/Regression &    Hidden States Output    & [CLS]         &   Entity Tokens \\
            Sequence Classification/Regression &    Pooling                 &  -            &   Max Pool.; Mean Pool.; Entity Start\\
            Sequence Classification/Regression &    Top Layer               & Linear Layer  &   Bi-LSTM  \\
            Token Classification & Tagging                 & BIO           &   BIOUL; IO \\
            Token Classification& Top Layer               & Linear Layer  &   Bi-LSTM  \\

\bottomrule
\end{tabular}
    \caption{Model Variants.}
    \label{tab:model_var}
\end{table}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\aiden{Added two tables for model choices. In general, we use CLS + Linear Layer as the standard model for sequence models and hidden states + Linear Layer for token classification models.@hoifung, In what format would you recommend organizing this?}
%\hoifung{Aiden/Rob: please insert fine-tuning model choice table} 


%\hoifung{representation; backprop; + archi: input - representation - task-spec - prediction}
%\hoifung{Seq len}
% \tristan{Would be nice to highlight which portion of this diagram is task-specific.}
% \hoifung{Good pt: it's basically implied as everything not "neural LM".}
% \tristan{Newer versions of the figure make this more clear.}

%%% rationale
Pretrained neural language models provide a unifying foundation for learning task-specific models. 
Given an input token sequence, the language model produces a sequence of vectors in the contextual representation. A task-specific prediction model is then layered on top to generate the final output for a task-specific application.
Given task-specific training data, we can learn the task-specific model parameters and refine the BERT model parameters by gradient descent using backpropragation.

Prior work on biomedical NLP often adopts different task-specific models and fine-tuning methods, which makes it difficult to understand the impact of an underlying pretrained language model on task performance. 
In this section, we review standard methods and common variants used for each task.
In our primary investigation comparing pretraining strategies, we fix the task-specific model architecture using the standard method identifed here, to facilitate a head-to-head comparison among the pretrained neural language models. 
Subsequently, we start with the same pretrained BERT model, and conduct additional investigation on the impact for the various choices in the task-specific models.
For prior biomedical BERT models, our standard task-specific methods generally lead to comparable or better performance when compared to their published results.
% \jianfeng{need to clarify: when we say we fix pretrained models or task-specific models, do we only fix the model architectures or fix the model parameters? For example, if we compare two pre-trained models, we need to fix the task-specific model architecture, but need to re-train the parameters of the task-specific models.}
% \hoifung{Yes, we only fix the model class, but not parameters. Tweak a couple words above - see if that helps?}
% \tristan{I can see this fix and I *think* it addresses the issue.}

\subsection{A General Architecture for Fine-Tuning Neural Language Models}

%Neural language models provide a solid foundation for a wide-range of NLP tasks. 
\autoref{fig:fine-tuning} shows a general architecture of fine-tuning neural language models for downstream applications. 
An input instance is first processed by a $\tt TransformInput$ module which performs task-specific transformations such as appending special instance marker (e.g., $\tt [CLS]$) or dummifying entity mentions for relation extraction.
The transformed input is then tokenized using the neural language model's vocabulary, and fed into the neural language model. Next, the contextual representation at the top layer is processed by a $\tt Featurizer$ module, and then fed into the $\tt Predict$ module to generate the final output for a given task. 

To facilitate a head-to-head comparison, we apply the same fine-tuning procedure for all BERT models and tasks. Specifically, we use cross-entropy loss for classification tasks and mean-square error for regression tasks. We conduct hyperparameter search using the development set based on task-specific metrics. Similarly to previous work, we jointly fine-tune the parameters of the task-specific prediction layer as well as the underlying neural language model.
%\chenghao{No sure whether backprop is widely understood outside machine learning.}

%\hoifung{Rob/Aiden: Do we use mini-batch?}
%\rob{Yes we use mini-batch, I have added in this detail at the start of section 6.2 next to your other comment}


%\xiaodong{For \autoref{fig:fine-tuning}, do we replace all the name of drugs with a specific placeholder? Tranform-input should only tokenize the text into sub-tokens, and then append [cls]/[sep] tokens. Should we align the color of highlighted for different entities, e.g. BLUE for GENE.}
%\hoifung{We want to separate the transform input from BERT vocab step. Also, if you add the special tokens to vocab, then the effect is same. Re coloring, yes, we're using blue for gene (KRAS) and red for drug (talazoparib).}
%\xiaodong{Thanks Hoifung. It seems that RE requires an extra step. How about we add a sub figure to compare with other tasks, which makes it less confusing.}
% \hoifung{Per our discussion, I'll tweak the figure and clarify in caption.}
%\tristan{Was this done? If so, can we remove these comments?}
%\hoifung{yes}


\subsection{Task-Specific Problem Formulation and Modeling Choices}

\begin{table}[h]
    \centering
\begin{tabular}{lll}
%\toprule
\specialrule{1pt}{1.5pt}{1.5pt}

            Task                    &  Problem Formulation     & Modeling Choices\\
\midrule
            NER                         & Token Classification  & Tagging Scheme, Classification Layer\\
            PICO                        & Token Classification  & Tagging Scheme, Classification Layer\\
            Relation Extraction         & Sequence Classification   & Entity/Relation Representation, Classification Layer\\
            Sentence Similarity         & Sequence Regression       & Sentence Representation, Regression Loss\\
            Document Classification     & Sequence Classification   & Document Representation, Classification Layer\\
            Question Answering          & Sequence Classification   & Question/Text Representation, Classification Layer\\
\specialrule{1pt}{1.5pt}{1.5pt}
%\bottomrule
\end{tabular}
    \caption{Standard NLP tasks and their problem formulations and modeling choices.}
    \label{tab:task_model_choices}
\end{table}

Many NLP applications can be formulated as a classification or regression task, wherein either individual tokens or sequences are the prediction target. Modeling choices usually vary in two aspects: the instance representation and the prediction layer. \autoref{tab:task_model_choices} presents an overview of the problem formulation and modeling choices for tasks we consider and detailed descriptions are provided below. For each task, we highlight the standard modeling choices with an asterisk~(*).


\paragraph{NER} Given an input text span (usually a sentence), the NER task seeks to recognize mentions of entities of interest. It is typically formulated as a sequential labeling task, where each token is assigned a tag to signify whether it is in an entity mention or not. The modeling choices primarily vary on the tagging scheme and classification method. $\tt BIO$ is the standard tagging scheme that classifies each token as the beginning of an entity ($\tt B$), inside an entity ($\tt I$), or outside ($\tt O$). The NER tasks in BLURB are only concerned about one entity type (in JNLPBA, all the types are merged into one). In the case when there are multiple entity types, the $\tt BI$ tags would be further divided into fine-grained tags for specific types. Prior work has also considered more complex tagging schemes such as $\tt BIOUL$, where $\tt U$ stands for the last word of an entity and $\tt L$ stands for a single-word entity. We also consider the simpler $\tt IO$ scheme that only differentiates between in and out of an entity. Classification is done using a simple linear layer or more sophisticated sequential labeling methods such as LSTM or conditional random field (CRF) \cite{Lafferty01conditionalrandom}.
%\chenghao{This is the first CRF.}

\begin{itemize}
    \item $\tt TransformInput$: returns the input sequence as is.
    \item $\tt Featurizer$: returns the BERT encoding of a given token.
    \item Tagging scheme: $\tt BIO$*; $\tt BIOUL$; $\tt IO$.
    \item Classification layer: linear layer*; LSTM; CRF.
\end{itemize}

\paragraph{PICO} Conceptually, evidence-based medical information extraction is akin to slot filling, as it tries to identify the PIO elements in an abstract describing a clinical trial. However, it can be formulated as a sequential tagging task like NER, by classifying tokens belonging to each element. A token may belong to more than one element, e.g., participant (P) and intervention (I).  
\begin{itemize}
    \item $\tt TransformInput$: returns the input sequence as is.
    \item $\tt Featurizer$: returns the BERT encoding of a given token.
    \item Tagging scheme: $\tt BIO$*; $\tt BIOUL$; $\tt IO$.
    \item Classification layer: linear layer*; LSTM; CRF.
\end{itemize}

\paragraph{Relation Extraction} Existing work on relation extraction tends to focus on binary relations. Given a pair of entity mentions in a text span (typically a sentence), the goal is to determine if the text indicates a relation for the mention pair. 
There are significant variations in the entity and relation representations. To prevent overfitting by memorizing the entity pairs, the entity tokens are often augmented with start/end markers or replaced by a dummy token. For featurization, the relation instance is either represented by a special $\tt [CLS]$ token, or by concatenating the mention representations. In the latter case, if an entity mention contains multiple tokens, its representation is usually produced by pooling those of individual tokens (max or average). For computational efficiency, we use padding or truncation to set the input length to 128 tokens for GAD and 256 tokens for ChemProt and DDI which contain longer input sequences.
\begin{itemize}
    \item $\tt TransformInput$: entity (dummification*; start/end marker; original); relation ($\tt [CLS]$*; original).
    \item $\tt Featurizer$: entity (dummy token*; pooling); relation ($\tt [CLS]$ BERT encoding*; concatenation of the mention BERT encoding).
    \item Classification layer: linear layer*; more sophisticated classifiers (e.g., MLP).
\end{itemize}

%\xiaodong{Should we explicitly write down TransformInput in line 606 in RE like line 616?}
%\hoifung{There are multiple dimensions of variations. What is used here is the succinct desc w/o enumerate many combos}


\paragraph{Sentence Similarity} The similarity task can be formulated as a regression problem to generate a normalized score for a sentence pair. By default, a special $\tt [SEP]$ token is inserted to separate the two sentences, and a special $\tt [CLS]$ token is prepended to the beginning to represent the pair. The BERT encoding of $\tt [CLS]$ is used to compute the regression score.
\begin{itemize}
    \item $\tt TransformInput$: $\tt [CLS]$ $S_1$ $\tt [SEP]$ $S_2$ $\tt [SEP]$, for sentence pair $S_1, S_2$.
    \item $\tt Featurizer$: $\tt [CLS]$ BERT encoding.
    \item Regression layer: linear regression.
\end{itemize}

\paragraph{Document Classification} For each text span and category (an abstract and a cancer hallmark in HoC), the goal is to classify whether the text belongs to the  category. By default, a $\tt [CLS]$ token is appended to the beginning of the text, and its BERT encoding is passed on by the $\tt Featurizer$ for the final classification, which typically uses a simple linear layer.
\begin{itemize}
    \item $\tt TransformInput$: $\tt [CLS]$ $D$ $\tt [SEP]$, for document $D$.
    \item $\tt Featurizer$: returns $\tt [CLS]$ BERT encoding.
    \item Classification layer: linear layer.
\end{itemize}

%\hoifung{Do we add [CLS]? Do we truncate?}

\paragraph{Question Answering} For the two-way (yes/no) or three-way (yes/maybe/no) question-answering task, the encoding is similar to the sentence similarity task. Namely, a $\tt [CLS]$ token is prepended to the beginning, followed by the question and reference text, with a $\tt [SEP]$ token to separate the two text spans. The $\tt [CLS]$ BERT encoding is then used for the final classification. For computational efficiency, we use padding or truncation to set the input length to 512 tokens.
\begin{itemize}
    \item $\tt TransformInput$: $\tt [CLS]$ $Q$ $\tt [SEP]$ $T$ $\tt [SEP]$, for question $Q$ and reference text $T$.
    \item $\tt Featurizer$: returns $\tt [CLS]$ BERT encoding. 
    \item Classification layer: linear layer.
\end{itemize}

% \xiaodong{In BERT, if it is a single sentence task, its input is transformed as [cls] s1 [sep]; while it is a two-sentence task, [cls] s1 [sep] s2 [sep].
% Line 612: why it is [cls] s1 [cls] s2? Line 620: it requires [sep] at the end of text; Line 630: it also needs a [sep] at the end.}
% \hoifung{Thanks! Fixed. }

%\hoifung{Double check: linear vs sigmod}
%\hoifung{More details; backprop strategies.}
%\hoifung{Aiden/Rob: Can you confirm if we always backprop all the way? - yes always all the way}

%%%%%%%%%%%%%%%%%%%%
\eat{
Prior work on biomedical NLP often adopts different task-specific models and fine-tuning methods, which makes it harder to conduct head-to-head comparison of the underlying pretrained language models. 
In this section, we enumerate the standard method and potential variants for each task.
In our main investigation comparing pretraining strategies, we fix the task-specific model to the standard one for each task, to facilitate a head-to-head comparison among the various pretrained BERT models. We perform a compact hyperparameter search for finetuning each model on each task, using learning rates 1e-5, 3e-5 and 5e-5 with a slanted triangular learning rate scheduler. For some tasks in-domain models performed better with less training than out-domain models, see \autoref{tab:task_model_choices} for the ranges of epochs corresponding to each task.
Subsequently, we fix the pretrained BERT model to the best one we find, and conduct additional investigation on the impact for the various choices in the task-specific models.
For the prior BERT models, our standard task-specific methods generally lead to comparable or better performance compared to their published results.



%We prepend input sentences with the \texttt{[CLS]} token and truncate inputs to 128 tokens. 
%The sentence pairs $(s_1, s_2)$ are labeled with an estimated similarity score in the range from 0 (no relation) to 4 (equivalent meanings). We use a preprocessed version of the BIOSSES corpus with fixed train, test, and development sets generated by \cite{peng2019transfer} and format the input to BERT models as \texttt{[CLS]} $s_1$ \texttt{[SEP]} $s_2$.



The sentence pairs $(s_1, s_2)$ are labeled with an estimated similarity score in the range from 0 (no relation) to 4 (equivalent meanings). We use a preprocessed version of the BIOSSES corpus with fixed train, test, and development sets generated by \cite{peng2019transfer} and format the input to BERT models as \texttt{[CLS]} $s_1$ \texttt{[SEP]} $s_2$.

Our experiments do not incorporate knowledge of the label hierarchy and jointly predict all 10 labels as individual sigmoidal outputs. Here we follow the data processing approach of \cite{peng2019transfer} and created matching train/dev/test splits.


%The BioASQ Task 7b corpus \cite{nentidis2019results} consists of multiple question answering tasks manually annotated by biomedical experts. It consists of yes/no, factoid, list, and summary questions, but we limit our experiments to the yes/no questions. Each question $q$ is paired with reference text $R$ containing multiple sentences from a PubMed abstract and a yes/no answer $a$. BioASQ's reference text is often very long, so we use a BERT input representation of \texttt{[CLS]q[SEP]R} and truncate the input length to 512 tokens. Predictions are made using a sigmoidal output in the range 0 (for "no") to 1 (for "yes").

%We also considered an alternative input representation for BioASQ that avoids truncating the reference text. In this experiment, we split the reference text $R$ into sentences $r_i$  and trained over tuples \texttt{(q, r\_i, a)} as separate training examples. During inference, we used the max of the individual sentence predictions as the final prediction for a given question with the interpretation that we expect the answer to these questions be "no" unless we see evidence that the answer is "yes" in one or more sentences. We found that this approach did not perform well and include its description here for posterity.
}
%%%%%%%%%%%%%%%%%%%%
